DSR: Towards Drone Image Super-Resolution

Despite achieving remarkable progress in recent years, single-image super-resolution methods are developed with several limitations. Specifically, they are trained on fixed content domains with certain degradations (whether synthetic or real). The priors they learn are prone to overfitting the training configuration. Therefore, the generalization to novel domains such as drone top view data, and across altitudes, is currently unknown. Nonetheless, pairing drones with proper image super-resolution is of great value. It would enable drones to fly higher covering larger fields of view, while maintaining a high image quality. To answer these questions and pave the way towards drone image super-resolution, we explore this application with particular focus on the single-image case. We propose a novel drone image dataset, with scenes captured at low and high resolutions, and across a span of altitudes. Our results show that off-the-shelf state-of-the-art networks witness a significant drop in performance on this different domain. We additionally show that simple fine-tuning, and incorporating altitude awareness into the network's architecture, both improve the reconstruction performance.

==> tables/color_correction.tex <==
\newcolumntype{A}{>{\centering}p{0.28\textwidth}}
\newcolumntype{B}{>{\centering}p{0.134\textwidth}}
\newcolumntype{C}{>{\centering\arraybackslash}p{0.134\textwidth}}
\begin{table}[tb]
    \centering
    \begin{tabular}{ABBBBC}
        \toprule
        Method                                              &10$m$ & 20$m$ & 30$m$  & 40$m$ & 50$m$ \\\hline
        Origin LR                                                   & 2.12/.7365 & 2.90/.7588 & 21.17/.7733 & 21.44/.7890 & 21.60/.7939  \\
        Histogram Match(HM)                                     & 23.74/.7598 & 24.59/.7814 & 25.04/\textcolor{red}{.7959} & 25.35/\textcolor{red}{.8079} & 25.39/.8109  \\
        Color Transfer(CT)                                         & 23.65/.7601 & 24.52/.7813 & 24.91/.7950 & 25.17/.8067 & 25.22/.8102  \\
        HM + CT                                                     & \textcolor{red}{23.80}/.7599 & \textcolor{red}{24.63}/.7809 & \textcolor{red}{25.06}/.7949 & \textcolor{red}{25.36}/.8071 & \textcolor{red}{25.42}/.8103  \\
        CT + HM                                                     & 23.77/\textcolor{red}{.7606} & \textcolor{red}{24.63}/\textcolor{red}{.7814} & \textcolor{red}{25.06}/.7954 & \textcolor{red}{25.36}/.8075 & \textcolor{red}{25.42}/.8107  \\
        \bottomrule
    \end{tabular}
    
    \begin{tabular}{ABBBBC}
        \toprule
        
        Method                                                & 70$m$  & 80$m$ & 100$m$  & 120$m$  & 140$m$ \\\hline
        Origin LR                                                   & 21.52/.8004 & 21.54/.8025 & 21.67/.8114 & 21.99/.8233 & 22.14/.8269 \\
        Histogram Match(HM)                                     & 25.63/\textcolor{red}{.8176} & 25.66/\textcolor{red}{.8192} & 25.87/.8287 & 26.03/\textcolor{red}{.8392} & 26.07/\textcolor{red}{.8420} \\
        Color Transfer(CT)                                         & 25.47/.8169 & 25.50/.8184 & 25.66/.8276 & 25.79/.8370 & 25.83/.8401 \\
        HM + CT                                                     & 25.67/.8171 & 25.70/.8185 & 25.92/.8285 & 26.08/.8386 & 26.12/.8417 \\
        CT + HM                                                     & \textcolor{red}{25.68}/.8174 & \textcolor{red}{25.71}/.8186 & \textcolor{red}{25.93}/\textcolor{red}{.8290} & \textcolor{red}{26.09}/.8387 & \textcolor{red}{26.13}/\textcolor{red}{.8420} \\
        \bottomrule
    \end{tabular}
    \caption{PSNR/SSIM between LR patches with different color correction methods and corresponding downsampled HR patches in our dataset. All results are calculated on the Y channel in the transformed YCbCr space. We highlight in red the best result.}
    \label{tab: color-matcing-dronesr}
\end{table}

==> tables/finetune-swinir.tex <==
\newcolumntype{A}{>{\centering}p{0.2\textwidth}}
\newcolumntype{B}{>{\centering}p{0.15\textwidth}}
\newcolumntype{C}{>{\centering\arraybackslash}p{0.15\textwidth}}
\begin{table}[ht]
    \centering
    \begin{tabular}{ABBBBC}
        \toprule
        Method & 10$m$ & 20$m$ & 30$m$ & 40$m$ & 50$m$ \\\hline
        
        Pretrained$^\ddagger$
        & 23.07/.7171
        & 23.17/.7151
        & 23.34/.7165
        & 23.78/.7305
        & 23.79/.7375
        \\
        
        Fine-tuned$^*$
        & 23.67/.7219
        & 23.73/.7162
        & 23.92/.7172
        & 24.36/.7350
        & 24.35/.7421
        \\
        
        \bottomrule
    \end{tabular}

    \begin{tabular}{ABBBBC}
        \toprule
        Method & 70$m$ & 80$m$ & 100$m$ & 120$m$ & 140$m$ \\\hline
    
        Pretrained$^\ddagger$
        & 24.00/.7497
        & 24.16/.7520
        & 24.27/.7615
        & 24.71/.7778
        & 24.64/.7815
        \\
        
        Fine-tuned$^*$
        & 24.61/.7570
        & 24.78/.7601
        & 24.88/.7684
        & 25.36/.7847
        & 25.28/.7897
        \\
        
        \hline
        \bottomrule
    \end{tabular}
    \caption{PSNR (\textit{dB})/SSIM results of the pretrained and fine-tuned SwinIR network on our DSR test set. $^\ddagger$The network is pretrained on Div2K. $^*$The network is fine-tuned on DSR using all altitudes.}
    \label{tab: fine-tune}
\end{table}


==> tables/finetune.tex <==
\begin{table}[bt]
    \tiny
    \setlength\tabcolsep{2.5pt}
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{\makecell[c]{PSNR/SSIM/LPIPS}}} & \multicolumn{10}{c|}{Test} \\\cline{3-12}
        \multicolumn{2}{|c|}{}          & 10$m$ & 20$m$ & 30$m$ & 40$m$ & 50$m$ & 70$m$ & 80$m$ & 100$m$ & 120$m$ & 140$m$ \\\hline 
        
        \multicolumn{2}{|c|}{Bicubic}   & \makecell[c]{23.12\\.7089\\.5769}%\\.1836 
                                        & \makecell[c]{22.69\\.6836\\.5959}%\\.1983
                                        &  \makecell[c]{23.39\\.6992\\.5836}%\\.1996
                                        &  \makecell[c]{24.25\\.7325\\.5694}%\\.1903
                                        &  \makecell[c]{24.41\\.7418\\.5727}%\\.1932
                                        &  \makecell[c]{24.14\\.7456\\.5633}%\\.1920
                                        &  \makecell[c]{24.16\\.7518\\.5584}%\\.1909
                                        &  \makecell[c]{24.27\\.7655\\.5572}%\.1875
                                        &  \makecell[c]{24.34\\.7668\\.5597}%\\.1883
                                        &  \makecell[c]{24.41\\.7724\\.5581}%\\.1872
                                        \\\hline
        
        \multicolumn{2}{|c|}{Pretrain} &  \makecell[c]{22.99\\.7111\\\textbf{.5402}}%\\.1946
                                        &  \makecell[c]{22.57\\.6871\\\textbf{.5592}}%\.2081
                                        &  \makecell[c]{23.32\\.7036\\\textbf{.5531}}%\.2073
                                        &  \makecell[c]{24.15\\.7361\\\textbf{.5451}}%\\.1983
                                        &  \makecell[c]{24.35\\\textbf{.7461}\\\textbf{.5504}}%\\.2001
                                        &  \makecell[c]{24.07\\\textbf{.7495}\\\textbf{.5448}}%\\.1991
                                        &  \makecell[c]{24.08\\\textbf{.7557}\\\textbf{.5408}}%\\.1980
                                        &  \makecell[c]{24.20\\\textbf{.7702}\\\textbf{.5400}}%\\.1940
                                        &  \makecell[c]{24.27\\\textbf{.7716}\\\textbf{.5428}}%\\.1943
                                        &  \makecell[c]{24.34\\.7771\\.5423}%\\.1935
                                        \\\hline
        
        \multirow{11}{*}{\rotatebox[origin=c]{90}{\hspace{-120pt} Fine-tune}}
         
        & All                           &  \makecell[c]{23.38\\.7118\\.5423}%\\.1984
                                        &  \makecell[c]{22.97\\.6869\\.5639}%\\.2140
                                        &  \makecell[c]{23.60\\.6998\\.5566}%\\.2142
                                        &  \makecell[c]{24.43\\.7336\\.5484}%\\.2051
                                        &  \makecell[c]{\textbf{24.58}\\.7404\\.5535}%\\.2066
                                        &  \makecell[c]{24.31\\.7457\\.5473}%\\.2045
                                        &  \makecell[c]{24.32\\.7519\\.5423}%\\.2028
                                        &  \makecell[c]{24.44\\.7655\\.5415}%\\.1985
                                        &  \makecell[c]{24.52\\.7669\\.5434}%\\.1988
                                        &  \makecell[c]{24.60\\.7733\\\textbf{.5421}}%\\.1974
                                        \\\cline{2-12}
                                        
        & 10$m$                           & \makecell[c]{\textbf{23.44}\\.7064\\.5526}%\\.2001
                                        & \makecell[c]{\textbf{23.01}\\.6805\\.5767}%\\.2164
                                        & \makecell[c]{\textbf{23.61}\\.6926\\.5691}%\\.2166
                                        & \makecell[c]{\textbf{24.45}\\.7280\\.5583}%\\.2065
                                        &  \makecell[c]{24.56\\.7335\\.5648}%\\.2087
                                        &  \makecell[c]{24.31\\.7386\\.5581}%\\.2070
                                        &  \makecell[c]{24.32\\.7445\\.5530}%\\.2055
                                        &  \makecell[c]{24.43\\.7565\\.5530}%\\.2023
                                        &  \makecell[c]{24.48\\.7571\\.5555}%\\.2028
                                        &  \makecell[c]{24.56\\.7635\\.5537}%\\.2016
                                        \\\cline{2-12}
                                        
        & 20$m$                           &  \makecell[c]{23.40\\.7092\\.5460}%\\.1992
                                        &  \makecell[c]{22.98\\.6837\\.5678}%\\.2150
                                        &  \makecell[c]{\textbf{23.61}\\.6964\\.5601}%\\.2152
                                        &  \makecell[c]{24.44\\.7311\\.5505}%\\.2056
                                        &  \makecell[c]{24.57\\.7372\\.5559}%\\.2074
                                        &  \makecell[c]{24.31\\.7423\\.5503}%\\.2056
                                        &  \makecell[c]{24.32\\.7484\\.5453}%\\.2041
                                        &  \makecell[c]{24.43\\.7609\\.5449}%\\.2005
                                        &  \makecell[c]{24.50\\.7618\\.5472}%\\.2009
                                        &  \makecell[c]{24.58\\.7683\\.5456}%\\.1997
                                        \\\cline{2-12}
                                        
        & 30$m$                           &  \makecell[c]{23.36\\.7097\\.5428}%\\.1985
                                        &  \makecell[c]{22.95\\.6844\\.5643}%\\.2139
                                        &  \makecell[c]{23.59\\.6975\\.5571}%\\.2143
                                        &  \makecell[c]{24.41\\.7315\\.5483}%\\.2050
                                        &  \makecell[c]{24.56\\.7382\\.5532}%\\.2066
                                        &  \makecell[c]{24.28\\.7435\\.5473}%\\.2046
                                        &  \makecell[c]{24.29\\.7494\\.5422}%\\.2031
                                        &  \makecell[c]{24.41\\.7627\\.5416}%\\.1990
                                        &  \makecell[c]{24.48\\.7637\\.5439}%\\.1994
                                        &  \makecell[c]{24.56\\.7702\\.5424}%\\.1980
                                        \\\cline{2-12}
                                        
        & 40$m$                           &  \makecell[c]{23.36\\.7106\\.5442}%\\.1986
                                        &  \makecell[c]{22.95\\.6854\\.5659}%\\.2141
                                        &  \makecell[c]{23.59\\.6983\\.5589}%\\.2144
                                        &  \makecell[c]{24.41\\.7322\\.5498}%\\.2051
                                        &  \makecell[c]{24.56\\.7390\\.5550}%\\.2067
                                        &  \makecell[c]{24.29\\.7444\\.5484}%\\.2045
                                        &  \makecell[c]{24.30\\.7503\\.5435}%\\.2031
                                        &  \makecell[c]{24.42\\.7639\\.5426}%\\.1988
                                        &  \makecell[c]{24.49\\.7651\\.5449}%\\.1991
                                        &  \makecell[c]{24.57\\.7718\\.5433}%\\.1976
                                        \\\cline{2-12}
                                        
        & 50$m$                           &  \makecell[c]{23.36\\.7114\\.5435}%\\.1982
                                        &  \makecell[c]{22.94\\.6861\\.5649}%\\.2138
                                        &  \makecell[c]{23.59\\.6990\\.5581}%\\.2142
                                        &  \makecell[c]{24.41\\.7330\\.5494}%\\.2049
                                        &  \makecell[c]{24.56\\.7395\\.5551}%\\.2066
                                        &  \makecell[c]{24.29\\.7449\\.5486}%\\.2045
                                        &  \makecell[c]{24.30\\.7508\\.5436}%\\.2030
                                        &  \makecell[c]{24.42\\.7644\\.5425}%\\.1987
                                        &  \makecell[c]{24.49\\.7656\\.5447}%\\.1991
                                        &  \makecell[c]{24.58\\.7723\\.5432}%\\.1977
                                        \\\cline{2-12}
                                        
        & 70$m$                           &  \makecell[c]{23.34\\.7133\\.5422}%\\.1985
                                        &  \makecell[c]{22.93\\.6884\\.5625}%\\.2137
                                        &  \makecell[c]{23.58\\.7012\\.5553}%\\.2140
                                        &  \makecell[c]{24.41\\.7347\\.5479}%\\.2049
                                        &  \makecell[c]{24.57\\.7414\\.5536}%\\.2067
                                        &  \makecell[c]{24.30\\.7470\\.5469}%\\.2045
                                        &  \makecell[c]{24.31\\.7529\\.5421}%\\.2029
                                        &  \makecell[c]{24.43\\.7667\\.5408}%\\.1987
                                        &  \makecell[c]{24.50\\.7679\\.5431}%\\.1989
                                        &  \makecell[c]{24.58\\.7743\\.5414}%\\.1975
                                        \\\cline{2-12}
                                        
        & 80$m$                           &  \makecell[c]{23.35\\.7131\\.5439}%\\.1974
                                        &  \makecell[c]{22.94\\.6880\\.5645}%\\.2128
                                        &  \makecell[c]{23.58\\.7011\\.5571}%\\.2132
                                        &  \makecell[c]{24.41\\.7344\\.5497}%\\.2041
                                        &  \makecell[c]{24.57\\.7415\\.5547}%\\.2058
                                        &  \makecell[c]{24.29\\.7465\\.5486}%\\.2038
                                        &  \makecell[c]{24.31\\.7527\\.5436}%\\.2020
                                        &  \makecell[c]{24.43\\.7662\\.5421}%\\.1979
                                        &  \makecell[c]{24.50\\.7676\\.5440}%\\.1981
                                        &  \makecell[c]{24.58\\.7741\\.5426}%\\.1967
                                        \\\cline{2-12}
                                        
        & 100$m$                          &  \makecell[c]{23.33\\.7134\\.5433}%\\.1975
                                        &  \makecell[c]{22.91\\.6885\\.5633}%\\.2128
                                        &  \makecell[c]{23.57\\.7016\\.5561}%\\.2130
                                        &  \makecell[c]{24.40\\.7348\\.5489}%\\.2040
                                        &  \makecell[c]{24.55\\.7418\\.5547}%\\.2057
                                        &  \makecell[c]{24.29\\.7469\\.5482}%\\.2037
                                        &  \makecell[c]{24.30\\.7532\\.5432}%\\.2019
                                        &  \makecell[c]{24.42\\.7672\\.5419}%\\.1975
                                        &  \makecell[c]{24.49\\.7688\\.5434}%\\.1976
                                        &  \makecell[c]{24.58\\.7753\\.5422}%\\.1961
                                        \\\cline{2-12}
                                        
        & 120$m$                          &  \makecell[c]{23.33\\.7130\\.5436}%\\.1972
                                        &  \makecell[c]{22.91\\.6882\\.5637}%\\.2125
                                        &  \makecell[c]{23.57\\.7018\\.5563}%\\.2127
                                        &  \makecell[c]{24.40\\.7347\\.5496}%\\.2039
                                        &  \makecell[c]{24.55\\.7419\\.5552}%\\.2055
                                        &  \makecell[c]{24.29\\.7472\\.5487}%\\.2034
                                        &  \makecell[c]{24.30\\.7535\\.5442}%\\.2018
                                        &  \makecell[c]{24.42\\.7674\\.5428}%\\.1973
                                        &  \makecell[c]{24.50\\.7690\\.5446}%\\.1974
                                        &  \makecell[c]{24.58\\.7753\\.5434}%\\.1961
                                        \\\cline{2-12}
                                        
        & 140$m$                          &  \makecell[c]{23.34\\\textbf{.7155}\\.5432}%\\.1967
                                        &  \makecell[c]{22.92\\\textbf{.6907}\\.5631}%\\.2118
                                        &  \makecell[c]{23.58\\\textbf{.7038}\\.5556}%\\.2121
                                        &  \makecell[c]{24.42\\\textbf{.7368}\\.5484}%\\.2032
                                        &  \makecell[c]{\textbf{24.58}\\.7438\\.5545}%\\.2050
                                        &  \makecell[c]{\textbf{24.32}\\.7492\\.5478}%\\.2028 
                                        &  \makecell[c]{\textbf{24.33}\\.7552\\.5431}%\\.2013
                                        &  \makecell[c]{\textbf{24.45}\\.7693\\.5419}%\\.1968 
                                        &  \makecell[c]{\textbf{24.53}\\.7710\\.5434}%\\.1969 
                                        &  \makecell[c]{\textbf{24.61}\\\textbf{.7772}\\.5422}%\\.1954
                                        \\\hline
    \end{tabular}
    \caption{Evaluation results of fine-tuned models. We evaluate the performance using PSNR, SSIM and LPIPS on the Y channel in the transformed YCbCr space. The best results are in bold.}
    \label{tab: fine-tune}
\end{table}

==> tables/gap.tex <==
\begin{table}[h]
    \setlength\tabcolsep{2.5pt}
    \tiny
    \centering
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Public} & \multicolumn{10}{c|}{Our} \\\cline{4-18}
        & & & Div2K & Set5 & Set14 & B100 & Urban100 & 10$m$ & 20$m$ & 30$m$ & 40$m$ & 50$m$ & 70$m$ & 80$m$ & 100$m$ & 120$m$ & 140$m$ \\\hline
        
        % \multirow{4}{*}{-}
        % & \multirow{4}{*}{-}
        % &PSNR & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        % &&GMSD & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\hline

        \multirow{4}{*}{Bicubic}
        & \multirow{4}{*}{-}
        &PSNR & 26.56 & 26.37 & 24.30 & 24.62 & 21.82 & 23.12 & 22.69 & 23.39 & 24.25 & 24.41 & 24.14 & 24.16 & 24.27 & 24.34 & 24.41 \\\cline{3-18}
        &&SSIM & 0.9593 & 0.7504 & 0.7065 & 0.6013 & 0.7722 & 0.7089 & 0.6836 & 0.6992 & 0.7325 & 0.7418 & 0.7456 & 0.7518 & 0.7655 & 0.7668 & 0.7724 \\\cline{3-18}
        &&LPIPS & 0.4731 & 0.4149 & 0.4963 & 0.5281 & 0.4851 & 0.5769 & 0.5959 & 0.5836 & 0.5694 & 0.5727 & 0.5633 & 0.5584 & 0.5572 & 0.5597 & 0.5581 \\\cline{3-18}
        &&GMSD & 0.1435 & 0.1469 & 0.1641 & 0.1565 & 0.1979 & 0.1836 & 0.1983 & 0.1996 & 0.1903 & 0.1932 & 0.1920 & 0.1909 & 0.1875 & 0.1883 & 0.1872 \\\hline\hline
        
        % \multirow{4}{*}{Bicubic}
        % & \multirow{4}{*}{-}
        % &PSNR & 26.56 & 26.37 & 24.30 & 24.62 & 21.82 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9593 & 0.7504 & 0.7065 & 0.6013 & 0.7722 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.4731 & 0.4149 & 0.4963 & 0.5281 & 0.4851 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1435 & 0.1469 & 0.1641 & 0.1565 & 0.1979 & - & - & - & - & - & - & - & - & - & - \\\hline\hline
        
        \multirow{4}{*}{EDSR~\cite{lim2017enhanced}} 
        & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        &PSNR & 28.27 & 28.91 & 26.07 & 25.80 & 23.76 & 22.95 & 22.52 & 23.27 & 24.07 & 24.29 & 23.98 & 23.99 & 24.11 & 24.17 & 24.24 \\\cline{3-18}
        &&SSIM & 0.9796 & 0.8581 & 0.7870 & 0.6657 & 0.8793 & 0.7099 & 0.6860 & 0.7027 & 0.7346 & 0.7455 & 0.7481 & 0.7542 & 0.7689 & 0.7700 & 0.7758 \\\cline{3-18}
        &&LPIPS & 0.3911 & 0.2959 & 0.4065 & 0.4498 & 0.3530 & 0.5435 & 0.5605 & 0.5525 & 0.5429 & 0.5472 & 0.5388 & 0.5343 & 0.5336 & 0.5364 & 0.5367 \\\cline{3-18}
        &&GMSD & 0.1031 & 0.0889 & 0.1181 & 0.1229 & 0.1391 & 0.1880 & 0.2013 & 0.2014 & 0.1927 & 0.1945 & 0.1947 & 0.1935 & 0.1895 & 0.1902 & 0.1896 \\\hline
        
        % \multirow{4}{*}{EDSR~\cite{lim2017enhanced}} 
        % & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        % &PSNR & 28.27 & 28.91 & 26.07 & 25.80 & 23.76 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9796 & 0.8581 & 0.7870 & 0.6657 & 0.8793 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3911 & 0.2959 & 0.4065 & 0.4498 & 0.3530 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1031 & 0.0889 & 0.1181 & 0.1229 & 0.1391 & - & - & - & - & - & - & - & - & - & - \\\hline
        
        \multirow{4}{*}{RDN~\cite{zhang2018residual}}
        & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        &PSNR & 28.20 & 28.73 & 26.06 & 25.75 & 23.62 & 22.96 & 22.53 & 23.28 & 24.09 & 24.30 & 24.00 & 24.00 & 24.12 & 24.18 & 24.25 \\\cline{3-18}
        &&SSIM & 0.9791 & 0.8540 & 0.7841 & 0.6626 & 0.8732 & 0.7100 & 0.6861 & 0.7029 & 0.7348 & 0.7456 & 0.7484 & 0.7544 & 0.7690 & 0.7702 & 0.7760 \\\cline{3-18}
        &&LPIPS & 0.3979 & 0.3010 & 0.4118 & 0.4556 & 0.3679 & 0.5455 & 0.5626 & 0.5540 & 0.5438 & 0.5481 & 0.5395 & 0.5351 & 0.5346 & 0.5372 & 0.5371 \\\cline{3-18}
        &&GMSD & 0.1050 & 0.0922 & 0.1195 & 0.1246 & 0.1442 & 0.1874 & 0.2008 & 0.2009 & 0.1924 & 0.1944 & 0.1944 & 0.1933 & 0.1894 & 0.1901 & 0.1893 \\\hline
        
        % \multirow{4}{*}{RDN~\cite{zhang2018residual}}
        % & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        % &PSNR & 28.20 & 28.73 & 26.06 & 25.75 & 23.62 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9791 & 0.8540 & 0.7841 & 0.6626 & 0.8732 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3979 & 0.3010 & 0.4118 & 0.4556 & 0.3679 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1050 & 0.0922 & 0.1195 & 0.1246 & 0.1442 & - & - & - & - & - & - & - & - & - & - \\\hline
        
        \multirow{4}{*}{RCAN~\cite{zhang2018image}}
        & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        &PSNR & 28.27 & 28.78 & 26.11 & 25.81 & 23.82 & 22.93 & 22.51 & 23.26 & 24.07 & 24.28 & 23.98 & 23.97 & 24.10 & 24.16 & 24.23 \\\cline{3-18}
        &&SSIM & 0.9795 & 0.8575 & 0.7867 & 0.6668 & 0.8814 & 0.7097 & 0.6858 & 0.7026 & 0.7345 & 0.7454 & 0.7482 & 0.7541 & 0.7687 & 0.7702 & 0.7758
        \\\cline{3-18}
        &&LPIPS & 0.3900 & 0.2971 & 0.4055 & 0.4488 & 0.3472 & 0.5430 & 0.5604 & 0.5520 & 0.5423 & 0.5466 & 0.5385 & 0.5347 & 0.5336 & 0.5367 & 0.5368 \\\cline{3-18}
        &&GMSD & 0.1031 & 0.0882 & 0.1178 & 0.1229 & 0.1373 & 0.1889 & 0.2021 & 0.2022 & 0.1934 & 0.1953 & 0.1952 & 0.1945 & 0.1903 & 0.1908 & 0.1902 \\\hline
        
        % \multirow{4}{*}{RCAN~\cite{zhang2018image}}
        % & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        % &PSNR & 28.27 & 28.78 & 26.11 & 25.81 & 23.82 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9795 & 0.8575 & 0.7867 & 0.6668 & 0.8814 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3900 & 0.2971 & 0.4055 & 0.4488 & 0.3472 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1031 & 0.0882 & 0.1178 & 0.1229 & 0.1373 & - & - & - & - & - & - & - & - & - & - \\\hline
        
        \multirow{4}{*}{ESRGAN~\cite{wang2018esrgan}}
        & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2K\\Bicubic downsample\\X4}}
        &PSNR & 26.35 & 26.66 & 24.53 & 24.01 & 22.25 & 22.78 & 22.37 & 23.13 & 23.91 & 24.14 & 23.81 & 23.80 & 23.94 & 23.95 & 24.01 \\\cline{3-18}
        &&SSIM & 0.9666 & 0.7976 & 0.7186 & 0.5890 & 0.8372 & 0.7070 & 0.6833 & 0.7000 & 0.7322 & 0.7431 & 0.7453 & 0.7515 & 0.7662 & 0.7667 & 0.7723 \\\cline{3-18}
        &&LPIPS & 0.3220 & 0.2700 & 0.3445 & 0.3637 & 0.3007 & 0.5316 & 0.5637 & 0.5569 & 0.5458 & 0.5520 & 0.5437 & 0.5356 & 0.5346 & 0.5394 & 0.5371 \\\cline{3-18}
        &&GMSD & 0.1155 & 0.1093 & 0.1289 & 0.1333 & 0.1476  & 0.1884 & 0.2015 & 0.2014 & 0.1924 & 0.1944 & 0.1943 & 0.1932 & 0.1894 & 0.1904 & 0.1902 \\\hline
    
        % \multirow{4}{*}{ESRGAN~\cite{wang2018esrgan}}
        % & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2K\\Bicubic downsample\\X4}}
        % &PSNR & 26.35 & 26.66 & 24.53 & 24.01 & 22.25 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9666 & 0.7976 & 0.7186 & 0.5890 & 0.8372 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3220 & 0.2700 & 0.3445 & 0.3637 & 0.3007 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1155 & 0.1093 & 0.1289 & 0.1333 & 0.1476  & - & - & - & - & - & - & - & - & - & - \\\hline
        
        \multirow{4}{*}{BSRNet~\cite{zhang2021designing}}
        & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2+WED+FFHQ\\Designed Degradation model\\X4}}
        &PSNR & 27.22 & 27.17 & 24.99 & 25.16 & 22.75 & 22.38 & 22.09 & 22.83 & 23.61 & 23.87 & 23.60 & 23.62 & 23.70 & 23.77 & 23.86 \\\cline{3-18}
        &&SSIM & 0.9651 & 0.7924 & 0.7309 & 0.6285 & 0.8269 & 0.7021 & 0.6818 & 0.6992 & 0.7293 & 0.7419 & 0.7472 & 0.7537 & 0.7678 & 0.7698 & 0.7762 \\\cline{3-18}
        &&LPIPS & 0.4573 & 0.3756 & 0.4761 & 0.5175 & 0.4387 & 0.5471 & 0.5584 & 0.5492 & 0.5415 & 0.5469 & 0.5406 & 0.5375 & 0.5361 & 0.5393 & 0.5399 \\\cline{3-18}
        &&GMSD & 0.1329 & 0.1259 & 0.1568 & 0.1531 & 0.1816 & 0.1935 & 0.2024 & 0.2034 & 0.1981 & 0.1993 & 0.1988 & 0.1980 & 0.1938 & 0.1945 & 0.1933 \\\hline
        
        % \multirow{4}{*}{BSRNet~\cite{zhang2021designing}}
        % & \multirow{4}{*}{-}
        % &PSNR & 27.22 & 27.17 & 24.99 & 25.16 & 22.75 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9651 & 0.7924 & 0.7309 & 0.6285 & 0.8269 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.4573 & 0.3756 & 0.4761 & 0.5175 & 0.4387 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1329 & 0.1259 & 0.1568 & 0.1531 & 0.1816 & - & - & - & - & - & - & - & - & - & - \\\hline
        
        % \multirow{4}{*}{SwinIR~\cite{liang2021swinir}}
        % & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        % &PSNR & 28.45 & 28.79 & 26.10 & 25.88 & 24.09 & 22.91 & 22.47 & 23.22 & 24.02 & 24.25 & 23.94 & 23.94 & 24.05 & 24.10 & 24.16 \\\cline{3-18}
        % &&SSIM & 0.9809 & 0.8630 & 0.7930 & 0.6727 & 0.8946 & 0.7095 & 0.6852 & 0.7019 & 0.7342 & 0.7452 & 0.7479 & 0.7539 & 0.7685 & 0.7694 & 0.7755 \\\cline{3-18}
        % &&LPIPS & 0.3816 & 0.2952 & 0.3996 & 0.4409 & 0.3335 & 0.5451 & 0.5610 & 0.5530 & 0.5436 & 0.5470 & 0.5393 & 0.5347 & 0.5342 & 0.5369 & 0.5373 \\\cline{3-18}
        % &&GMSD & 0.0989 & 0.0879 & 0.1164 & 0.1202 & 0.1291 & 0.1902 & 0.2035 & 0.2034 & 0.1945 & 0.1961 & 0.1961 & 0.1951 & 0.1909 & 0.1917 & 0.1911 \\\hline
        
        \multirow{4}{*}{SwinIR~\cite{liang2021swinir}} 
        &&PSNR & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        &&SSIM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        &&LPIPS & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        &&GMSD & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\hline
        
        
        % \multirow{4}{*}{SwinIR~\cite{liang2021swinir}} 
        % &&PSNR & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        % &&LPIPS & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        % &&GMSD & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\hline
        
        \multirow{4}{*}{NLSN~\cite{Mei_2021_CVPR}}
        & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X4}}
        &PSNR & 28.31 & 28.91 & 26.15 & 25.86 & 24.00 & 22.95 & 22.52 & 23.27 & 24.08 & 24.30 & 23.99 & 24.00 & 24.12 & 24.18 & 24.25 \\\cline{3-18}
        &&SSIM & 0.9796 & 0.8607 & 0.7891 & 0.6689 & 0.8862 & 0.7099 & 0.6859 & 0.7027 & 0.7347 & 0.7456 & 0.7484 & 0.7545 & 0.7692 & 0.7703 & 0.7760 \\\cline{3-18}
        &&LPIPS & 0.3893 & 0.2917 & 0.4037 & 0.4433 & 0.3418 & 0.5440 & 0.5605 & 0.5518 & 0.5423 & 0.5459 & 0.5379 & 0.5333 & 0.5328 & 0.5355 & 0.5356 \\\cline{3-18}
        &&GMSD & 0.1026 & 0.0868 & 0.1164 & 0.1210 & 0.1330 & 0.1887 & 0.2020 & 0.2021 & 0.1929 & 0.1950 & 0.1948 & 0.1937 & 0.1896 & 0.1902 & 0.1897 \\\hline
        
        % \multirow{4}{*}{SwinIR(X4)~\cite{liang2021swinir}} 
        % & \multirow{4}{*}{real}
        % &PSNR & 25.41 & 24.31 & 23.44 & 23.71 & 21.16 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9402 & 0.6958 & 0.6842 & 0.5838 & 0.7936 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3873 & 0.3311 & 0.4130 & 0.4177 & 0.3624 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1384 & 0.1415 & 0.1580 & 0.1517 & 0.1829 & - & - & - & - & - & - & - & - & - & - \\\hline
        
        % \multirow{4}{*}{SwinIR(X4)[large]~\cite{liang2021swinir}}
        % & \multirow{4}{*}{-}
        % &PSNR & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\cline{3-18}
        % &&GMSD & - & - & - & - & - & - & - & - & - & - & - & - & - & - & -  \\\hline\hline
        
        \multirow{4}{*}{DASR~\cite{wang2021unsupervised}}
        & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2K\\Different Degradation model\\X4}}
        &PSNR & 27.97 & 28.25 & 25.83 & 25.64 & 23.36 & 23.03 & 22.60 & 23.32 & 24.14 & 24.35 & 24.05 & 24.07 & 24.18 & 24.25 & 24.31 \\\cline{3-18}
        &&SSIM & 0.9775 & 0.8447 & 0.7769 & 0.6590 & 0.8633 & 0.7106 & 0.6866 & 0.7030 & 0.7350 & 0.7457 & 0.7487 & 0.7547 & 0.7692 & 0.7706 & 0.7763 \\\cline{3-18}
        &&LPIPS & 0.4067 & 0.3100 & 0.4218 & 0.4614 & 0.3864 & 0.5484 & 0.5658 & 0.5561 & 0.5454 & 0.5490 & 0.5407 & 0.5364 & 0.5356 & 0.5382 & 0.5381 \\\cline{3-18}
        &&GMSD & 0.1087 & 0.0972 & 0.1232 & 0.1259 & 0.1503 & 0.1871 & 0.2007 & 0.2012 & 0.1923 & 0.1944 & 0.1940 & 0.1931 & 0.1892 & 0.1897 & 0.1888 \\\hline
        
        % \multirow{4}{*}{DASR~\cite{wang2021unsupervised}}
        % & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2K\\Degradation model\\X4}}
        % &PSNR & 27.97 & 28.25 & 25.83 & 25.64 & 23.36 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9775 & 0.8447 & 0.7769 & 0.6590 & 0.8633 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.4067 & 0.3100 & 0.4218 & 0.4614 & 0.3864 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1087 & 0.0972 & 0.1232 & 0.1259 & 0.1503  & - & - & - & - & - & - & - & - & - & -  \\\hline
        
        % \multirow{4}{*}{ArbRCAN~\cite{wang2021learning}} 
        % & \multirow{4}{*}{\makecell[c]{Div2K\\Bicubic downsample\\X50/9}}
        % &PSNR & 28.41 & 28.81 & 26.30 & 25.86 & 24.04 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&SSIM & 0.9802 & 0.8528 & 0.7878 & 0.6658 & 0.8842 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&LPIPS & 0.3913 & 0.2963 & 0.4062 & 0.4499 & 0.3481 & - & - & - & - & - & - & - & - & - & - \\\cline{3-18}
        % &&GMSD & 0.1020 & 0.0906 & 0.1150 & 0.1230 & 0.1343 & - & - & - & - & - & - & - & - & - & - \\\hline
        
    \end{tabular}
    \caption{Evaluation results of SOTA SR model on public and our dataset. Our dataset has a fixed scale factor of 50/9, and all public datasets are downsampled according to this scale factor using the MATLAB bicubic kernel function. For the networks that are not pre-trained on our scale factor, we upsampled the networks' output to fit our scale factor. We evaluate the results using PSNR, SSIM, LPIPS, and GMSD on the Y channel in the transformed YCbCr space.}
    \label{tab:domain gap}
\end{table}

% \begin{table}[h]
%     \tiny
%     \centering
%     \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
%         \hline
%         \multirow{2}{*}{Method} & \multirow{2}{*}{Train set} & \multirow{2}{*}{Metric} & \multicolumn{5}{c|}{Public} & \multicolumn{10}{c|}{Our} \\\cline{4-18}
%         & & & Div2K & Set5 & Set14 & B100 & Urban100 & 10m & 20m & 30m & 40m & 50m & 70m & 80m & 100m & 120m & 140m \\\hline 
        
%         \multirow{4}{*}{Bicubic}
%         & \multirow{4}{*}{-}
%         &PSNR & 26.56 & 26.37 & 24.30 & 24.62 & 21.82 & 21.25 & 22.90 & 24.24 & 24.35 & 24.71 & 24.94 & 24.91 & 24.92 & 24.79 & 24.64 \\\cline{3-18}
%         &&SSIM & 0.9593 & 0.7504 & 0.7065 & 0.6013 & 0.7722 & 0.5720 & 0.5919 & 0.6431 & 0.6519 & 0.6735 & 0.7012 & 0.7038 & 0.7172 & 0.7284 & 0.7189 \\\cline{3-18}
%         &&LPIPS & 0.4731 & 0.4149 & 0.4963 & 0.5281 & 0.4851 & 0.6398 & 0.6315 & 0.6171 & 0.6220 & 0.6096 & 0.5996 & 0.5995 & 0.5949 & 0.5925 & 0.5927 \\\cline{3-18}
%         &&GMSD & 0.1435 & 0.1469 & 0.1641 & 0.1565 & 0.1979 & 0.2060 & 0.1995 & 0.1877 & 0.1919 & 0.1861 & 0.1823 & 0.1843 & 0.1833 & 0.1838 & 0.1860 \\\hline\hline
        
%         \multirow{4}{*}{DASR~\cite{wang2021unsupervised}}
%         & \multirow{4}{*}{\makecell[c]{Div2K+Flickr2K\\Degradation model\\X4}}
%         &PSNR & 27.97 & 28.25 & 25.83 & 25.64 & 23.36 & 21.09 & 22.72 & 24.05 & 24.17 & 24.54 & 24.77 & 24.71 & 24.73 & 24.59 & 24.43 \\\cline{3-18}
%         &&SSIM & 0.9775 & 0.8447 & 0.7769 & 0.6590 & 0.8633 & 0.5688 & 0.5884 & 0.6392 & 0.6489 & 0.6703 & 0.6979 & 0.6997 & 0.7142 & 0.7255 & 0.7153 \\\cline{3-18}
%         &&LPIPS & 0.4067 & 0.3100 & 0.4218 & 0.4614 & 0.3864 & 0.6043 & 0.6019 & 0.5928 & 0.5979 & 0.5877 & 0.5784 & 0.5781 & 0.5731 & 0.5713 & 0.5724 \\\cline{3-18}
%         &&GMSD & 0.1087 & 0.0972 & 0.1232 & 0.1259 & 0.1503 & 0.2100 & 0.2024 & 0.1901 & 0.1940 & 0.1880 & 0.1846 & 0.1875 & 0.1865 & 0.1872 & 0.1894 \\\hline
        
%     \end{tabular}
%     \caption{Evaluation results of SOTA SR model on public and our dataset. Our dataset has a fixed scale factor of 50/9, and all public datasets are downsampled according to this scale factor using the MATLAB bicubic kernel function. For the networks that are not pre-trained on our scale factor, we upsampled the networks' output to fit our scale factor. We evaluate the results using PSNR, SSIM, LPIPS, and GMSD on the Y channel in the transformed YCbCr space. To eliminate the effect of color mismatch, histogram matching with corresponding HR images is applied on our LR images before sending them into the networks.}
%     \label{tab:domain-gap-histogram-matcing}
% \end{table}



==> tables/misalignment_realsr.tex <==
\begin{table}[hbt]
    \centering
    \begin{tabular}{c|ccc}
        \toprule
        Scale factor & x2           & x3            & x4  \\
        PSNR/SSIM    & 32.25/0.9318 & 30.20/0.9105  & 29.7484/0.9113\\
        \bottomrule
    \end{tabular}
    \caption{PSNR/SSIM between LR images in the RealSR (\cite{cai2019ntire,cai2019toward}) dataset and corresponding downscaled HR images. All results are calculated on the Y channel in the transformed YCbCr space.}
    \label{tab: color-matcing-realsr}
\end{table}
